Vote'n'Rank: Revision of Benchmarking with Social Choice Theory

The development of state-of-the-art systems in different applied areas of machine learning (ML) is driven by benchmarks, which have shaped the paradigm of evaluating generalisation capabilities from multiple perspectives. Although the paradigm is shifting towards more fine-grained evaluation across diverse tasks, the delicate question of how to aggregate the performances has received particular interest in the community. In general, benchmarks follow the unspoken utilitarian principles, where the systems are ranked based on their mean average score over task-specific metrics. Such aggregation procedure has been viewed as a sub-optimal evaluation protocol, which may have created the illusion of progress. This paper proposes Vote'n'Rank, a framework for ranking systems in multi-task benchmarks under the principles of the social choice theory. We demonstrate that our approach can be efficiently utilised to draw new insights on benchmarking in several ML sub-fields and identify the best-performing systems in research and development case studies. The Vote'n'Rank's procedures are more robust than the mean average while being able to handle missing performance scores and determine conditions under which the system becomes the winner.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> parts/2_1_related_work_NLP.tex <==
%\paragraph{Aggregation methods and principles.}
%The recent research has addressed these limitations, introducing novel aggregation methods and principles. 


%HULK \cite{zhou2021hulk} explores compute requirements for a system to reach a pre-defined performance level.  \cite{henderson2020towards} advocate for reporting averaged performance together with practical hardware-oriented metrics to better account for real-life scenarios. 
%\cite{ethayarajh2020utility} put forward new requirements for user-specific rankings and propose the  micro-economic \textit{utility}-based framework to account for LM's performance and costs simultaneously. For that matter, DynaBench systems user preferences by estimating how much of performance can user sacrifice to reduce compute costs (i.e. marginal rate of substitution with respect to performance)  \citep{dynaboard}. Inspired by statistical testing, \citep{peyrard2021better} evaluate the Bradley–Terry (BT) model which leverages the instance-level pairing of metric scores. Experiments on four tasks and 18 evaluation metrics show that paired aggregation mechanisms such as BT are more robust alternatives to the mean and median.

% bayesian system to evaluate reliability of rankings \cite{rodriguez-etal-2021-evaluation}


==> parts/2_2_related_work_SCT.tex <==
\paragraph{Applications of social choice theory.}
%The works that are the closest to ours and based on social choice theory are two recent works by \citep{choudhury2021linguistically},\citep{colombo2022best}.

%\citep{choudhury2021linguistically} propose several strategies to evaluate multilingual language models based on the normative principles of efficiency and fairness, although in a different way from this work. 
%In particular, they emphasize Rawlsian principle, where one should select the model which maximizes the minimum performance (with respect to languages, or tasks, or both). However, this principle requires homogeneous criteria such as accuracy for different languages, while we take it a step further and focus on ranking rules and heterogeneous data. 

%\citep{colombo2022best} relies on a ranking aggregation procedure to evaluate systems on multi-tasks benchmarks. The authors adopt Kemeny consensus aggregation procedure that satisfies the Condorcet criterion. Although these recent works shed some light on how to utilize a voting rule and stems from the social choice theory, none of them has been \textbf{...hmmm study diversity of rules ans aggregation procedures in depth? do not use weighting? idk... }. Therefore, the \textsc{Vote'n'Rank} framework can be viewed as an extension and unification of the previous works on evaluation of NLP models and social choice theory.


% \paragraph{Applications of social choice theory.}
% A detailed and contemporary overview of the field of computational social choice is provided in \cite{moulin_2016}.



==> parts/3_3_framework_upd.tex <==
% \textbf{Definitions.} We adopt the conceptual definitions from the social choice theory to the objectives of selecting the best-performing system and ranking a set of systems as follows: {\it (i) a voter} is a task in a given benchmark, {\it (ii) an alternative} is a system candidate, and {\it (iii) a criterion} is the task performance score.

% \textbf{Objectives.} Suppose we have a set $M$ of alternatives $m \in \{m_1,\ldots, m_{|M|}\}$ from the benchmark including a set $T$ of voters $t \in \{t_1,\ldots,t_{|T|}\}$ and the corresponding criteria $S = \{ s_{mt} \}_{m = 1, t = 1}^{m = |M|, t = |T|} $. Given that, we pursue two main objectives of the aggregation procedure  $\sigma$, $\sigma: S \mapsto (M,\succ_{\sigma})$: {\it (i)} to select the best performing alternative $m^{*}$, so that there is no alternative $\hat{m}, \hat{m} \succ_{\sigma} m^{*}$, and {\it (ii)} to rank the alternatives in the descending order according to $\sigma$ values, so that $m_i \succ_{\sigma} m_j$. 

%\textbf{Settings.} 
The framework supports three settings of performing the aggregation objectives. \autoref{fig:ex_leaderboard} illustrates a toy example of the benchmark result aggregation. The toy benchmark has three evaluated alternatives and consists of seven voters grouped by the task, e.g. natural language inference, text classification, and question answering (QA).

\begin{enumerate}[leftmargin=2.em,label=\Alph*,itemsep=0pt]
\item \underline{Basic aggregation}: the aggregation procedure is applied to the leaderboard as it is.
\item \underline{Weighted aggregation}: each voter in the group is assigned a group weight equal to $1/|T_{group}|$. The blue group weights are $1/3$, and the orange and the violet group weights are $1/2$. Each group contributes equally to the final ranking, regardless of the number of voters. 
\item \underline{Two-step aggregation}: each voter group is treated as a standalone leaderboard. We independently apply an aggregation procedure to each voter group and conduct an interim ranking, depicted as ``elector'' in the example. Next, we aggregate the group-wise rankings by applying the same procedure one more time and achieve the final ranking.
\end{enumerate}





==> parts/checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{Our work aims at re-thinking benchmarking strategies for evaluating ML systems. We have described the societal impact in Appendix D.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{Our paper does not make a theoretical contribution.} %No, we do not present new theoretical results
	\item Did you include complete proofs of all theoretical results?
    \answerNA{Our paper does not make a theoretical contribution.} % No, we do not present new theoretical results
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide  all data and experiments as supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Case Study 4 relies on the default GLUE splits and default fine-tuning and evaluation hyperparameters under the HuggingFace library. The other studies re-use publicly available results.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, we report error bars in supplemental material.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We provide detailed information on the computational resources.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, systems) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{The license information can be found in the corresponding references. We have mentioned the license of the published code and experiment materials in our README.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide  all data and experiments as supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{No, all benchmark data is publicly available.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{No, the ethical considerations may be discussed in the original papers, specifically StereoSet, Winobias, and CrowS-Pairs.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}


==> remainders.tex <==

%In some cases it is impossible to calculate certain metrics for some systems. For instance, this can happen if training a system on a particular dataset requires too many computational resources, or when it is not possible to figure out the level of human performance on a task.

%Ranking via averaging scores is unable to handle such cases. If a system misses a score on a task, then one can not calculate the average score of this system across all tasks. Thus, in that case there is nothing better to do than to discard all columns with at least one missing value.

%\begin{wrapfigure}{r}{0.5\textwidth}
%    \centering
%    \input{tables/winner_ex1}
%    \caption{The results of the winner selection for the \textsc{GLUE}, \textsc{SuperGLUE}, and \textsc{VALUE} benchmarks. \underline{Notations}: \human=\textsc{Human}; \ernie=\textsc{ERNIE}; \johnson=\textsc{T5+UDG}; \smileman=\textsc{DeBERTa+CLEVER}; \textsc{craig.starr}=?.}
%\end{wrapfigure}

% Other developments include evaluation of cross-lingual transfer \citep{hu2020xtreme,liang-etal-2020-xglue}, domain-specific problems \citep{mehri2020dialoglue,lu2021codexglue}, language models' linguistic competence \citep{gauthier-etal-2020-syntaxgym}.

% %Benchmarks are used to measure progress in different areas of ML research. To this end, benchmarks take a form of a leaderboard, so that models are scored across multiple tasks. With a few exceptions, benchmarks follow {\it utilitarian} principles, under which average performance scores are maximised. The best model is determined according to the highest average score. Such evaluation protocol has inevitably led to undesirable consequences, notably, SoTA-chasing behavior and incremental improvements at the cost of compute resources. 

%Based on research in {\it Social Choice Theory}, we introduce a framework to aggregate models' scores on a leaderboard. We implement a variety of theoretically sound aggregation procedures:  scoring rules, scoring elimination rules, positional rules, and majority-relation based rules. 
%We demonstrate the usefulness of our framework with four case studies in the NLP area: (i) we re-rank existing NLP leaderboards (e.g. GLUE, SuperGLUE, VALUE), (ii) we explore, under what conditions, a language model becomes dominant, (iii) we show that our frameworks is capable of handling missing scores, and (iv) we present a multifaceted evaluation, in which downstream performance, social bias, and compute usage are brought together to score a language model. Overall, our framework provides with meaningful insights into model comparison and benchmarking. 

%\paragraph{Language Model Evaluation}. LMs' evaluation protocols are classified into two major categories: \textit{intrinsic} methods, which assess the LM's representations independent of any specific task, and \textit{extrinsic} approaches, which estimate downstream performance.  Intrinsic approaches encompass unsupervised techniques to (i) estimate how well an LM fits a held-out set (i.e perplexity) and matches statistical tendencies of natural text \citep{meister-cotterell-2021-language}; (ii) probe for linguistic structures, captured by LMs' constituents, by training light-weighted classifiers on top of latent representations  \cite{conneau-kiela-2018-senteval,sahin-etal-2020-linspector} or using didicated unsupervised techniques \citep{hewitt-manning-2019-structural}. A recent line of research suggests functional tests in form of cloze questions of minimal contrastive pairs to measure commonsense understanding and world knowledge \cite{petroni-etal-2019-language},  social biases \citep{nangia-etal-2020-crows}, linguistic competence \citep{warstadt-etal-2020-blimp-benchmark}, reasoning abilities \cite{talmor-etal-2020-olmpics}.  Extrinsic downstream applications include supervised text classification \cite{minaee2021deep}, named entity recognition \cite{lothritz-etal-2020-evaluating}, question answering \cite{rajpurkar-etal-2016-squad}. Recent works explore the abilities of LM's to perform in resource-savvy  zero- and few-shot setups \cite{yin-etal-2019-benchmarking,zheng2021fewnlu}, transfer learning across domains \cite{lee2020biobert} and languages \cite{hu2020xtreme,liang-etal-2020-xglue}, generalize to unseen and out-of-domain inputs  \cite{morris-etal-2020-textattack}. The variety of evaluation protocols and aspects makes it impossible to develop a single performance metric. This motivates the need for benchmarks, accounting for diverse tasks. This work highlights the need for procedures to aggregate benchmarking results.


% In scenarios (i)-(iii) arithmetic averaging of all features chooses RoBERTa-base as the best model. Geometric averaging of all features chooses DistilBERT-base as the best model.

% Scenario (i):  Distilled models appear occupy the top positions.  XX out XX rules select DistilRoBERTa-base, followed by DistilBERT-base (XX out XX).

% Scenario (ii):  XX out XX rules select DistilBERT-base, X rules select  DeBERTa-base and ALBERT-base.

% Scenario (iii): XX out XX rules select DistilBERT-base, XX rules select ALBERT-base, XX rules select BERT-base,  DistilRoBERTa-base and DeBERTa-base are selected one time each.

% Table \ref{table:two_step_borda} shows the model metrics aggregated via Borda count in scenario (iii) with equal weights assigned to each criteria group. All the models in the table are ranked according to their final order.
%% CS3
%A natural question that arises when discussing ranking methods capable of dealing with missing values is how much credence can be given to them. Will the ranking change drastically if we omit data in one of the leaderboard table cells?
%We compared the majority-relation-based Copeland method and the mean ranking. For that, we conducted experiments on the GLUE, SuperGLUE and VALUE benchmarks.

%For the range of possible number $N$ of missing values in the leaderboard, we did the following.

%First, we constructed rankings using both methods on data without missing values. Then we randomly chose $N$ cells in the GLUE table and replaced them with missing values.

%We then obtained a top-7 system ranking using the Copeland method, taking missing values into account, and calculated the Spearman correlation between that ranking and the Copeland ranking on the original data. The same procedure was done for Minimax method. Similarly, we ranked the systems via averaging, filling in the missing cells with column-wise medians, and calculated the Spearman correlation between this ranking and the ranking of systems on original data.


% ALBERT, which is neither the most powerful, nor the most efficient, is ranked the first. DistilBERT compensates low performance with high efficiency and low exposure to social bias, and thus comes the second. DeBERTa, though outperforming all other models on GLUE tasks, is the heaviest and the least efficient of all, so it is ranked the fifth.

% Other possible scenarios: (iv) use weights.

% Analysis: correlation with GLUE-only evaluation?



%We treat a leaderboard as a single voter; the model is considered as an alternative, and the downstream task as a criterion. 

% There is a multitude of voting rules. What is best voting rule to choose depends on the particular scenario we are working in. We  discuss the rules we use for ranking our models in Section~\ref{sec:background}. Particular voting rules include (1) the \emph{plurality voting rule}, where each voter names her favourite candidate, candidates with the largest number of votes win, and if two or more candidates get the highest score, the winner is chosen using a \emph{tie-breaking rule}, (2) \emph{Condorcet voting rules}, where each of the $n$ voters has a ranking of all $m$ candidates, a candidate $c$ wins a \emph{pairwise election} against candidate $d$ if more than half of the voters rank $c$ above $d$, and a candidate is said to be a \emph {Condorcet winner} if she wins in all pairwise elections she participates in, and (3) the \emph{Borda voting rule}, where a \emph{scoring rule} for an election with $m$ candidates is given by a vector $(s_1, \ldots, s_m)$, $s_1 \ge \ldots \ge s_m$, each candidate gets $s_i= m-i$ points from each voter who ranks her $i$-th, and the candidate with the \emph{maximum number of points} wins.



% здесь должно быть описание свойств правил, их сфера примения в экономике и других областях
% здесь нужно сделать заметку о терминологии: критерий –  задача / оценка модели, альтернатива – модель, тоже можно провести аналогии с более очевидными применениями аппарата 
% нужно дописать, какие требования выдвигаются к критериям / значениям критериев 
% здесь описаны не все реализованные правила: ещё есть k-Approval, Dowdall, q-паретовские, Minimax, Dogson, Schulze, ещё один вариант Copeland, победитель Кондорсе. Они все тут: https://amethyst-lettuce-a57.notion.site/10c046c3178c4b6083705f55a015539d?v=b1e18b1c53c944d9a553b3d4cae5ae6c


%As shown in \ref{subsection:reranking-benchmarks}, our framework allows us to assign weights to the criteria, and to rank systems according to those weights. The choice of weights vector can be determined by the needs of the researcher choosing the system, and reflect their priorities in system performance.

%Suppose there are $M$ systems, evaluated on $T$ task.  \textsc{Vote'n'Rank} inputs a leaderboard, i.e. the scores $S = \{ s_{mt} \}_{m = 1, t = 1}^{m = M, t = T} $ of the systems $m \in \{m_1,\ldots, m_M\}$ on tasks $t \in \{t_1,\ldots,t_T\}$ and applies aggregation procedures.
%Two main objectives of an aggregation procedure $\sigma$, $\sigma: S \mapsto (M,\succ_{\sigma})$ are: (i) to select the best performing system $m^{*}$, so that there is no system $\hat{m}, \hat{m} \succ m^{*}$, (ii) to rank the systems in descending order according to $\alpha$ values, so that $m_i \succ_{\sigma} m_j$. 


%multiple ways of running aggregation procedures. We aim at take into account not only tasks individually, but also groups of tasks and multifaceted evaluation, in which criteria are not only downstream performance, but also computer usage. The Figure \ref{fig:ex_leaderboard} exemplifies these setups. 

%There are three systems and three groups of tasks in the example leaderboard. The blue group consists of three tasks, the orange and the violet groups consist of two tasks each. The following are three ways to aggregate grouped tasks:

==> tables/cs2.tex <==
\begin{tabular}{cccc}
    \toprule
    \textbf{Benchmark} & \textsc{GLUE} & \textsc{SGLUE} & \textsc{VALUE} \\
    \midrule
    \boldmath{$N_p/N_n$} & 9/88 & 10/12 & 3/3 \\
    \bottomrule
 \end{tabular}


==> tables/ethics_cs4_res.tex <==
\begin{tabular}{lrrrr}
\toprule
{} & anti\_crows\_score & stereoset\_intra\_icat & stereoset\_inter\_icat & winobias\_acc\_difference \\
model\_name  &   &  &  & \\
\midrule
distilbert-base-uncased & 0.4098 & 0.6998 & 0.7528 &   0.9981 \\
bert-base-uncased  & 0.4138 & 0.7279 & 0.6700 &   0.9552 \\
roberta-base & 0.3773 & 0.6750 & 0.3995 &   0.9609 \\
albert-base-v2   & 0.4410 & 0.6901 & 0.7770 &   0.9924 \\
deberta-base & 0.5159 & 0.4248 & 0.4035 &   0.9867 \\
gpt2   & 0.4317 & 0.6975 & 0.6490 &   0.9255 \\
distilroberta-base & 0.3687 & 0.6833 & 0.6247 &   0.9861 \\
\bottomrule
\end{tabular}

==> tables/glue_cs4_res.tex <==
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
{} & wnli.eval\_accuracy & cola.eval\_matthews\_correlation & stsb.eval\_pearson & stsb.eval\_spearmanr & rte.eval\_accuracy & mrpc.eval\_accuracy & mrpc.eval\_f1 & sst2.eval\_accuracy & qnli.eval\_accuracy & qqp.eval\_accuracy & qqp.eval\_f1 & mnli.eval\_accuracy & mnli-mm.eval\_accuracy \\
model\_name & & & & & & & & & & & & & \\
\midrule
distilbert-base-uncased & 54.6 & 53.9 & 87.1 & 86.8 & 62.9 & 84.7 & 89.6 & 90.9 & 89.2 & 90.4 & 87.1 & 82.2 & 82.3 \\
bert-base-uncased & 42.5 & 59.0 & 89.7 & 89.3 & 69.7 & 85.8 & 90.0 & 92.9 & 91.5 & 91.2 & 88.2 & 84.4 & 84.9 \\
roberta-base & 56.3 & 60.4 & 90.6 & 90.4 & 76.0 & 89.1 & 92.1 & 94.1 & 92.5 & 91.5 & 88.7 & 87.5 & 87.2 \\
distilroberta-base & 51.5 & 56.1 & 86.9 & 86.7 & 64.5 & 84.0 & 88.7 & 91.8 & 90.9 & 90.9 & 87.8 & 84.0 & 84.3 \\
albert-base-v2 & 54.1 & 57.1 & 90.8 & 90.4 & 77.5 & 87.6 & 91.0 & 91.8 & 91.0 & 90.6 & 87.4 & 84.4 & 84.6 \\
deberta-base & 56.3 & 62.9 & 91.1 & 90.8 & 72.6 & 89.8 & 92.7 & 94.5 & 92.8 & 91.6 & 88.7 & 87.9 & 87.9 \\
gpt2 & 47.6 & 41.3 & 86.0 & 86.0 & 66.7 & 79.7 & 86.3 & 92.0 & 89.0 & 90.1 & 86.8 & 82.4 & 83.1 \\
\bottomrule
\end{tabular}

==> tables/spearman_cs3.tex <==
\begin{table}
  \caption{Spearman correlation $\times 100\%$ between rankings with a different ratio of missing values. Results are averaged over 100 runs.}
  \label{table:spearman}
  \centering
    \begin{tabular}{lrrrrrrrrrr}
    \toprule
    $\%$ missing &     0  &    10 &    20 &    30 &    40 &    50 &    60 &    70 &    80 &    90 \\
    \midrule
    AM     &  100.0 &  99.1 &  98.4 &  97.6 &  96.8 &  95.6 &  94.2 &  91.9 &  86.8 &  72.1 \\
    Copeland &  100.0 &  99.8 &  99.5 &  99.2 &  98.8 &  98.0 &  96.9 &  94.1 &  88.5 &  72.8 \\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/winners2.tex <==
%\begin{table}[th!]
%    \centering
%    \scriptsize
%    \setlength{\tabcolsep}{4pt}

\begin{tabular}{ccccccccccc}
    \toprule
    \textbf{Benchmark} & $\sigma^{am}$& $\sigma^{gm}$ & \textbf{Copeland} & \textbf{Minimax} & \textbf{Plurality} & \textbf{Dowdall} & \textbf{Borda} & \textbf{Threshold} & \textbf{Baldwin} & \textbf{Condorcet} \\
    \midrule
    %$\sigma^{am}$& \erniewinner & \erniewinner & \xmark/\sherlock  \\
    %$\sigma^{gm}$ &\erniewinner & \erniewinner & \xmark/\sherlock \\
    %\textbf{Copeland} & \erniewinner & \human & \human/\sherlock \\
    %\textbf{Minimax} & \erniewinner & \erniewinner \human & \human/\sherlock \\
    %\textbf{Plurality} & \erniewinner \human & \human & \xmark/\sherlock \\
    %\textbf{Dowdall} & \erniewinner & \human & \xmark/\sherlock \\
    %\textbf{Borda} & \erniewinner & \erniewinner & \xmark/\sherlock \\ 
    %\textbf{Threshold} & \oscarwinner & \johnsonwinner & \xmark/\sherlock \\
    %\textbf{Baldwin} & \erniewinner & \erniewinner \human & \xmark/\sherlock \\ 
    %\textbf{Condorcet} & \erniewinner & \xmark & \human/\sherlock \\
    \bottomrule
\end{tabular}
%    \label{winners_cs1}
%\end{table}
